Efficient evaluation of risk allocations

Expectations of marginals conditional on the total risk of a portfolio are crucial in risk-sharing and allocation. However, computing these conditional expectations may be challenging, especially in critical cases where the marginal risks have compound distributions or when the risks are dependent. We introduce a generating function method to compute these conditional expectations. We provide efficient algorithms to compute the conditional expectations of marginals given the total risk for a portfolio of risks with lattice-type support. We show that the ordinary generating function of unconditional expected allocations is a function of the multivariate probability generating function of the portfolio. The generating function method allows us to develop recursive and transform-based techniques to compute the unconditional expected allocations. We illustrate our method to large-scale risk-sharing and risk allocation problems, including cases where the marginal risks have compound distributions, where the portfolio is composed of dependent risks, and where the risks have heavy tails, leading in some cases to computational gains of several orders of magnitude. Our approach is useful for risk-sharing in peer-to-peer insurance and risk allocation based on Euler's rule.

==> code/pareto-plots.tex <==
\resizebox{0.25\textwidth}{!}{
	\begin{tikzpicture}
		\begin{axis}[
			xlabel={$x$},
			xmax = 60,
			ylabel={$\Pr(E[X_1 \vert S] \leq x)$},
			title = {$X_1, \alpha_1 = 1.3, \lambda_1 = 3$},
			%				enlargelimits=false,
			]
			\addplot [mark = none, thick, color = black] table[x="V1",y="V2", col sep = comma]{data/pareto1.csv};
			\addplot [mark = none, thick, color = blue, dotted] table[x="V1",y="V4", col sep = comma]{data/pareto3.csv};
			\addplot [mark = none, thick, color = blue, dashed] table[x="V1",y="V4", col sep = comma]{data/pareto100.csv};
			\addplot [mark = none, thick, color = blue, dashdotted] table[x="V1",y="V4", col sep = comma]{data/pareto1000.csv};
			\addplot [thick, green] coordinates {(9.201219,0)(9.201219,1)};
			
		\end{axis}
\end{tikzpicture}}
\resizebox{0.25\textwidth}{!}{
	\begin{tikzpicture}
		\begin{axis}[
			xlabel={$x$},
			xmax = 60,
			ylabel={$\Pr(E[X_2 \vert S] \leq x)$},
			title = {$X_2, \alpha_2 = 1.6, \lambda_2 = 6$},
			%				enlargelimits=false,
			]
			\addplot [mark = none, thick, color = black] table[x="V1",y="V3", col sep = comma]{data/pareto1.csv};
			\addplot [mark = none, thick, color = blue, dotted] table[x="V2",y="V4", col sep = comma]{data/pareto3.csv};
			\addplot [mark = none, thick, color = blue, dashed] table[x="V2",y="V4", col sep = comma]{data/pareto100.csv};
			\addplot [mark = none, thick, color = blue, dashdotted] table[x="V2",y="V4", col sep = comma]{data/pareto1000.csv};
			\addplot [thick, green] coordinates {(9.908447,0)(9.908447,1)};
			
		\end{axis}
\end{tikzpicture}}
\resizebox{0.25\textwidth}{!}{
	\begin{tikzpicture}
		\begin{axis}[
			xlabel={$x$},
			xmax = 60,
			ylabel={$\Pr(E[X_3 \vert S] \leq x)$},
			title = {$X_3, \alpha_3 = 1.9, \lambda_3 = 9$},
			%				enlargelimits=false,
			]
			\addplot [mark = none, thick, color = black] table[x="V1",y="V4", col sep = comma]{data/pareto1.csv};
			\addplot [mark = none, thick, color = blue, dotted] table[x="V3",y="V4", col sep = comma]{data/pareto3.csv};
			\addplot [mark = none, thick, color = blue, dashed] table[x="V3",y="V4", col sep = comma]{data/pareto100.csv};
			\addplot [mark = none, thick, color = blue, dashdotted] table[x="V3",y="V4", col sep = comma]{data/pareto1000.csv};
			\addplot [thick, green] coordinates {(9.988156,0)(9.988156,1)};
			
		\end{axis}
\end{tikzpicture}}
\resizebox{0.2\textwidth}{!}{
	\begin{tikzpicture} 
		\begin{axis}[%
			hide axis,
			enlargelimits=false,
			xmin=0,
			xmax=10,
			ymin=0,
			ymax=10,
			legend style={draw=white,legend cell align=left, at={(1, 1)}, 
			}
			]
			\addlegendimage{thick, black}
			\addlegendentry{$n = 1$};
			\addlegendimage{thick, blue, dotted}
			\addlegendentry{$n = 3$};
			\addlegendimage{thick, blue, dashed}
			\addlegendentry{$n = 100$};
			\addlegendimage{thick, blue, dashdotted}
			\addlegendentry{$n = 1000$};
			\addlegendimage{thick, green}
			\addlegendentry{Expected value};
		\end{axis}
\end{tikzpicture}}

